Simplify Node-RED For End User Development in SeismoCloud

Networks of IoT devices often require configuration and definition of behavior by the final user. Node-RED is a flow-based programming platform commonly used for End User Development, but it requires networking and protocols skills in order to be efficiently used. We add a level of abstraction to Node-RED nodes in order to allow non-skilled users to configure and control networks of IoT devices and online services. We applied such abstractions to the SeismoCloud application for earthquake monitoring.

==> sidebar.tex <==

\vspace{1pc}

  \fbox{%
    \begin{minipage}{0.925\textwidth}
      \textbf{Node-RED architecture} \\
      \\
      %\textbf{Nodes:} black-boxes with zero or one input and zero or more outputs. \\
      %\\
      %\textbf{Flow:} collection of nodes, possibly linked together. Usually a flow groups nodes for a specific purpose (e.g. room light control) \\
      %\\
      Node-RED user can drag and drop nodes into one or more flows (group of nodes for specific purposes, e.g. room light control), link the output of a node to the input of another node allowing a message ``produced'' by a node to be ``consumed'' by linked one (which, in turns, can output another message).
    \end{minipage}}
    
